Automated quality assessment using appearance-based simulations and hippocampus segmentation on low-field paediatric brain MR images

Understanding the structural growth of paediatric brains is a key step in the identification of various neuro-developmental disorders. However, our knowledge is limited by many factors, including the lack of automated image analysis tools, especially in Low and Middle Income Countries from the lack of high field MR images available. Low-field systems are being increasingly explored in these countries, and, therefore, there is a need to develop automated image analysis tools for these images. In this work, as a preliminary step, we consider two tasks: 1) automated quality assurance and 2) hippocampal segmentation, where we compare multiple approaches. For the automated quality assurance task a DenseNet combined with appearance-based transformations for synthesising artefacts produced the best performance, with a weighted accuracy of 82.3%. For the segmentation task, registration of an average atlas performed the best, with a final Dice score of 0.61. Our results show that although the images can provide understanding of large scale pathologies and gross scale anatomical development, there still remain barriers for their use for more granular analyses.

==> references.tex <==
@article{Hesse2022,
title = {Subcortical segmentation of the fetal brain in 3D ultrasound using deep learning},
journal = {NeuroImage},
volume = {254},
pages = {119117},
year = {2022},
doi = {https://doi.org/10.1016/j.neuroimage.2022.119117},
author = {Linde S. Hesse and Moska Aliasi and Felipe Moser and Monique C. Haak and Weidi Xie and Mark Jenkinson and Ana I.L. Namburete},
}

@article{hafiz2023se,
  title={SE-MD: a single-encoder multiple-decoder deep network for point cloud reconstruction from 2D images},
  author={Hafiz, Abdul Mueed and Bhat, Rouf Ul Alam and Parah, Shabir Ahmad and Hassaballah, M},
  journal={Pattern Analysis and Applications},
  volume={26},
  number={3},
  pages={1291--1302},
  year={2023},
  publisher={Springer}
}

@article{torchio2021,
   title = {TorchIO: a Python library for efficient loading, preprocessing, augmentation and patch-based sampling of medical images in deep learning},
   journal = {Computer Methods and Programs in Biomedicine},
   pages @article{perez-garcia_torchio_2021,
   title = {TorchIO: a Python library for efficient loading, preprocessing, augmentation and patch-based sampling of medical images in deep learning},
   journal = {Computer Methods and Programs in Biomedicine},
   pages = {106236},
   year = {2021},
   issn = {0169-2607},
   doi = {https://doi.org/10.1016/j.cmpb.2021.106236},
   url = {https://www.sciencedirect.com/science/article/pii/S0169260721003102},
   author = {P{\'e}rez-Garc{\'i}a, Fernando and Sparks, Rachel and Ourselin, S{\'e}bastien},
pages = {106236},
   year = {2021},
   issn = {0169-2607},
   doi = {https://doi.org/10.1016/j.cmpb.2021.106236},
   url = {https://www.sciencedirect.com/science/article/pii/S0169260721003102},
   author = {P{\'e}rez-Garc{\'i}a, Fernando and Sparks, Rachel and Ourselin, S{\'e}bastien},
}

@inproceedings{lin2017focal,
  title={Focal loss for dense object detection},
  author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2980--2988},
  year={2017}
}

@article{Moser2022,
title = {BEAN: Brain Extraction and Alignment Network for 3D Fetal Neurosonography},
journal = {NeuroImage},
volume = {258},
pages = {119341},
year = {2022},
doi = {https://doi.org/10.1016/j.neuroimage.2022.119341},
author = {Felipe Moser and Ruobing Huang and Bartłomiej W. Papież and Ana I.L. Namburete}
}

@InProceedings{Venturini2020,
author="Venturini, Lorenzo
and Papageorghiou, Aris T.
and Noble, J. Alison
and Namburete, Ana I. L.",
title="Multi-task CNN for Structural Semantic Segmentation in 3D Fetal Brain Ultrasound",
booktitle="Medical Image Understanding and Analysis",
year="2020",
pages="164--173",
}

@article{Dinsdale2021,
  title={Challenges for machine learning in clinical translation of big data imaging studies},
  author={Nicola K. Dinsdale and Emma Bluemke and Vaanathi Sundaresan and Mark Jenkinson and Stephen Smith and Ana I. L. Namburete},
  journal={Neuron},
  year={2021},
  volume={110},
  pages={3866-3881},
  url={https://api.semanticscholar.org/CorpusID:235829550}
}

@inproceedings{Ganin2015,
author = {Ganin, Yaroslav and Lempitsky, Victor},
title = {Unsupervised Domain Adaptation by Backpropagation},
year = {2015},
booktitle = {Proceedings of the 32nd International Conference on International Conference on Machine Learning - Volume 37},
pages = {1180–1189},
numpages = {10},
series = {ICML'15}
}

@InProceedings{Sun2016,
author="Sun, Baochen
and Saenko, Kate",
title="Deep CORAL: Correlation Alignment for Deep Domain Adaptation",
booktitle="Computer Vision -- ECCV 2016 Workshops",
year="2016",
pages="443--450",
doi="$10.1007/978-3-319-49409-8_35$"
}

@InProceedings{Liang2020,
  title = 	 {Do We Really Need to Access the Source Data? {S}ource Hypothesis Transfer for Unsupervised Domain Adaptation},
  author =       {Liang, Jian and Hu, Dapeng and Feng, Jiashi},
  booktitle = 	 {Proceedings of the 37th International Conference on Machine Learning},
  pages = 	 {6028--6039},
  year = 	 {2020},
  volume = 	 {119},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {13--18 Jul},
  publisher =    {PMLR},
  url = 	 {https://proceedings.mlr.press/v119/liang20a.html},
}

@InProceedings{Dinsdale2023,
    author    = {Dinsdale, Nicola K and Jenkinson, Mark and Namburete, Ana IL},
    title     = {SFHarmony: Source Free Domain Adaptation for Distributed Neuroimaging Analysis},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {11494-11505}
}

@article{Bateson2022,
title = {Source-free domain adaptation for image segmentation},
journal = {Medical Image Analysis},
volume = {82},
pages = {102617},
year = {2022},
issn = {1361-8415},
doi = {https://doi.org/10.1016/j.media.2022.102617},
author = {Mathilde Bateson and Hoel Kervadec and Jose Dolz and Hervé Lombaert and Ismail {Ben Ayed}}
}

@inproceedings{Wang2021,
title={Tent: Fully Test-Time Adaptation by Entropy Minimization},
author={Dequan Wang and Evan Shelhamer and Shaoteng Liu and Bruno Olshausen and Trevor Darrell},
booktitle={International Conference on Learning Representations},
year={2021},
}

@article{Namburete2023,
author = {Namburete, Ana and Papież, Bartłomiej and Fernandes, Michelle and Wyburd, Madeleine and Hesse, Linde and Moser, Felipe and Cheikh Ismail, Leila and Gunier, Robert and Squier, Waney and Ohuma, Eric and Carvalho, Maria and Jaffer, Yasmin and Gravett, Michael and Wu, Qingqing and Lambert, Ann and Winsey, Adele and Restrepo-Méndez, María and Bertino, Enrico and Purwar, Manorama and Kennedy, Stephen},
year = {2023},
month = {10},
pages = {},
title = {Normative spatiotemporal fetal brain maturation with satisfactory development at 2 years},
volume = {623},
journal = {Nature},
doi = {10.1038/s41586-023-06630-3}
}

@article{Dinsdale2022,
title = {STAMP: Simultaneous Training and Model Pruning for low data regimes in medical image segmentation},
journal = {Medical Image Analysis},
volume = {81},
pages = {102583},
year = {2022},
doi = {https://doi.org/10.1016/j.media.2022.102583},
author = {Nicola K. Dinsdale and Mark Jenkinson and Ana I.L. Namburete},
}

@inproceedings{Molchanov2017,
  author       = {Pavlo Molchanov and
                  Stephen Tyree and
                  Tero Karras and
                  Timo Aila and
                  Jan Kautz},
  title        = {Pruning Convolutional Neural Networks for Resource Efficient Inference},
  booktitle    = {5th International Conference on Learning Representations, {ICLR} 2017},
  year         = {2017},
}

@article{papageorghiou2018intergrowth,
  title={The INTERGROWTH-21st fetal growth standards: toward the global integration of pregnancy and pediatric care},
  author={Papageorghiou, Aris T and Kennedy, Stephen H and Salomon, Laurent J and Altman, Douglas G and Ohuma, Eric O and Stones, William and Gravett, Michael G and Barros, Fernando C and Victora, Cesar and Purwar, Manorama and others},
  journal={American journal of obstetrics and gynecology},
  volume={218},
  number={2},
  pages={S630--S640},
  year={2018},
}

@article{Dinsdale2021Harm,
title = {Deep learning-based unlearning of dataset bias for MRI harmonisation and confound removal},
journal = {NeuroImage},
volume = {228},
pages = {117689},
year = {2021},
doi = {https://doi.org/10.1016/j.neuroimage.2020.117689},
author = {Nicola K. Dinsdale and Mark Jenkinson and Ana I.L. Namburete}
}

@article{perez-garcia_torchio_2021,
   title = {TorchIO: a Python library for efficient loading, preprocessing, augmentation and patch-based sampling of medical images in deep learning},
   journal = {Computer Methods and Programs in Biomedicine},
   pages = {106236},
   year = {2021},
   doi = {https://doi.org/10.1016/j.cmpb.2021.106236},
   author = {P{\'e}rez-Garc{\'i}a, Fernando and Sparks, Rachel and Ourselin, S{\'e}bastien},
}

@article{Karani2021,
title = {Test-time adaptable neural networks for robust medical image segmentation},
journal = {Medical Image Analysis},
volume = {68},
pages = {101907},
year = {2021},
doi = {https://doi.org/10.1016/j.media.2020.101907},
author = {Neerav Karani and Ertunc Erdil and Krishna Chaitanya and Ender Konukoglu},
}

@article{Janouskova2024,
title = {Single Image Test-Time Adaptation for Segmentation},
journal = {ArXiv},
year = {2023},
doi = {https://arxiv.org/abs/2309.14052},
author = {Klara Janouskova and Tamir Shor and Chaim Baskin and Jiri Matas},
}

@article{Malinger2020,
  title={ISUOG Practice Guidelines (updated): sonographic examination of the fetal central nervous system. Part 1: performance of screening examination and indications for targeted neurosonography},
  author={Malinger, G and Paladini, D and Haratx, K and Monteagudo, A and Pulu, G and Timor-Tritsch, IE},
  journal={Ultrasound Obstet Gynecol},
  volume={56},
  pages={476--484},
  year={2020}
}

@article{yeung2024implicitvol,
    title={Sensorless Volumetric Reconstruction of Fetal Brain Freehand Ultrasound Scans 
           with Deep Implicit Representation},
    author={Yeung, Pak-Hei and Hesse, Linde and Aliasi, Moska and Haak, Monique 
            and Xie, Weidi and Namburete, Ana IL and others},
    journal={Medical Image Analysis},
    volume={94},
    pages={103147},
    year={2024},
    publisher={Elsevier}
  }

@inproceedings{Wyburd2020cortical,
  title={Cortical plate segmentation using CNNs in 3D fetal ultrasound},
  author={Wyburd, Madeleine K and Jenkinson, Mark and Namburete, Ana IL},
  booktitle={Annual Conference on Medical Image Understanding and Analysis},
  pages={56--68},
  year={2020},
  organization={Springer}
}


@InProceedings{HyperMorph,
author="Hoopes, Andrew
and Hoffmann, Malte
and Fischl, Bruce
and Guttag, John
and Dalca, Adrian V.",
title="HyperMorph: Amortized Hyperparameter Learning for Image Registration",
booktitle="Information Processing in Medical Imaging",
year="2021"
}

@article{Hesse2022,
title = {Subcortical segmentation of the fetal brain in 3D ultrasound using deep learning},
journal = {NeuroImage},
volume = {254},
pages = {119117},
year = {2022},
doi = {https://doi.org/10.1016/j.neuroimage.2022.119117},
author = {Linde S. Hesse and Moska Aliasi and Felipe Moser and Monique C. Haak and Weidi Xie and Mark Jenkinson and Ana I.L. Namburete},
}

@InProceedings{Ronneberger2015,
author="Ronneberger, Olaf
and Fischer, Philipp
and Brox, Thomas",
title="U-Net: Convolutional Networks for Biomedical Image Segmentation",
booktitle="Medical Image Computing and Computer-Assisted Intervention -- MICCAI 2015",
year="2015"
}

@article{balboni2022,
	title = {The impact of transfer learning on 3D deep learning convolutional neural network segmentation of the hippocampus in mild cognitive impairment and Alzheimer disease subjects},
	volume = {43},
	issn = {1097-0193},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/hbm.25858},
	doi = {10.1002/hbm.25858},
	pages = {3427--3438},
	number = {11},
    year={2022},
	journaltitle = {Human Brain Mapping},
	author = {Balboni, Erica and Nocetti, Luca and Carbone, Chiara and Dinsdale, Nicola and Genovese, Maurilio and Guidi, Gabriele and Malagoli, Marcella and Chiari, Annalisa and Namburete, Ana I. L. and Jenkinson, Mark and Zamboni, Giovanna},
}

@inproceedings{huang2017densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4700--4708},
  year={2017}
}

@article{patenaude2011,
	title = {A Bayesian model of shape and appearance for subcortical brain segmentation},
	volume = {56},
	issn = {1053-8119},
	url = {https://www.sciencedirect.com/science/article/pii/S1053811911002023},
	doi = {10.1016/j.neuroimage.2011.02.046},
	pages = {907--922},
	number = {3},
	journaltitle = {{NeuroImage}},
	shortjournal = {{NeuroImage}},
	author = {Patenaude, Brian and Smith, Stephen M. and Kennedy, David N. and Jenkinson, Mark},
	urldate = {2023-08-27},
	date = {2011-06-01},
	keywords = {Bayesian, Classification, Segmentation, Shape model, Subcortical structures},
}

@article{billot2023,
	title = {{SynthSeg}: Segmentation of brain {MRI} scans of any contrast and resolution without retraining},
	volume = {86},
	issn = {1361-8415},
	url = {https://www.sciencedirect.com/science/article/pii/S1361841523000506},
	doi = {10.1016/j.media.2023.102789},
	shorttitle = {{SynthSeg}},
	pages = {102789},
	journaltitle = {Medical Image Analysis},
	shortjournal = {Medical Image Analysis},
	author = {Billot, Benjamin and Greve, Douglas N. and Puonti, Oula and Thielscher, Axel and Van Leemput, Koen and Fischl, Bruce and Dalca, Adrian V. and Iglesias, Juan Eugenio},
	urldate = {2023-08-27},
	date = {2023-05-01},
	keywords = {{CNN}, Contrast and resolution invariance, Domain randomisation, Segmentation},
}

@article{Bateson2022,
title = {Source-free domain adaptation for image segmentation},
journal = {Medical Image Analysis},
volume = {82},
pages = {102617},
year = {2022},
issn = {1361-8415},
doi = {https://doi.org/10.1016/j.media.2022.102617},
author = {Mathilde Bateson and Hoel Kervadec and Jose Dolz and Hervé Lombaert and Ismail {Ben Ayed}}
}

@article{fischl2002,
	title = {Whole brain segmentation: automated labeling of neuroanatomical structures in the human brain},
	volume = {33},
	issn = {0896-6273},
	doi = {10.1016/s0896-6273(02)00569-x},
	shorttitle = {Whole brain segmentation},
	pages = {341--355},
	number = {3},
	journaltitle = {Neuron},
	shortjournal = {Neuron},
	author = {Fischl, Bruce and Salat, David H. and Busa, Evelina and Albert, Marilyn and Dieterich, Megan and Haselgrove, Christian and van der Kouwe, Andre and Killiany, Ron and Kennedy, David and Klaveness, Shuna and Montillo, Albert and Makris, Nikos and Rosen, Bruce and Dale, Anders M.},
	date = {2002-01-31},
	pmid = {11832223},
	keywords = {Aged, Alzheimer Disease, Brain, Brain Mapping, Female, Humans, Magnetic Resonance Imaging, Male, Reproducibility of Results},
}

@article{lecun2015deep,
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={nature},
  volume={521},
  number={7553},
  pages={436--444},
  year={2015},
  publisher={Nature Publishing Group UK London}
}


@article{thyreau2018,
	title = {Segmentation of the hippocampus by transferring algorithmic knowledge for large cohort processing},
	volume = {43},
	issn = {1361-8415},
	url = {https://www.sciencedirect.com/science/article/pii/S1361841517301597},
	doi = {10.1016/j.media.2017.11.004},
	pages = {214--228},
	journaltitle = {Medical Image Analysis},
	shortjournal = {Medical Image Analysis},
	author = {Thyreau, Benjamin and Sato, Kazunori and Fukuda, Hiroshi and Taki, Yasuyuki},
	urldate = {2024-07-29},
	date = {2018-01-01},
}

@article{jenkinson2002,
title = {Improved Optimization for the Robust and Accurate Linear Registration and Motion Correction of Brain Images},
journal = {NeuroImage},
volume = {17},
number = {2},
pages = {825-841},
year = {2002},
issn = {1053-8119},
doi = {https://doi.org/10.1006/nimg.2002.1132},
url = {https://www.sciencedirect.com/science/article/pii/S1053811902911328},
author = {Mark Jenkinson and Peter Bannister and Michael Brady and Stephen Smith},
keywords = {accuracy, affine transformation, global optimization, motion correction, multimodal registration, multiresolution search, robustness},

}

@article{Biobank,
title = {UK Biobank: An Open Access Resource for Identifying the Causes of a Wide Range of Complex Diseases of Middle and Old Age},
journal = {PLOS Medicine},
volume = {12},
number = {3},
year = {2015},
doi = {https://doi.org/10.1371/journal.pmed.1001779},
author = {Cathie Sudlow and John Gallacher and Naomi Allen and Valerie Beral and Paul Burton and John Danesh and  Paul Downey and Paul Elliott and Jane Green and Martin Landray and Bette Liu and Paul Matthews and Giok Ong and  Jill Pell and Alan Silman and Alan Young and  Tim Sprosen and Tim Peakman and Rory Collins}
}


@article{LISA2024,
    author = {Lepore, N. and Linguraru, M. G. and Deoni, S. and Tanedo, J. and Rouhi, R. and Zanjal, S. and Tapp, A. and Nelson, M. and  Lecurieux Lafayette S., and Nankabirwa, V.} ,
    title = {Low field pediatric brain magnetic resonance Image Segmentation and quality Assurance - 27th International Conference on Medical Image Computing and Computer Assisted Intervention (MICCAI 2024)},
    journal = {Zenodo},
    year = {2024},
    doi = {https://doi.org/10.5281/zenodo.10992222}
}

@article{Dinsdale2021,
  title={Challenges for machine learning in clinical translation of big data imaging studies},
  author={Nicola K. Dinsdale and Emma Bluemke and Vaanathi Sundaresan and Mark Jenkinson and Stephen Smith and Ana I. L. Namburete},
  journal={Neuron},
  year={2021},
  volume={110},
  pages={3866-3881},
  url={https://api.semanticscholar.org/CorpusID:235829550}
}

@article{Anand2012,
    author = {Anand KS and Dhikav V} ,
    title = {Hippocampus in health and disease: An overview.},
    journal = {Indian Acad Neurol.},
    year = {2012} 
}


@article{Ahmad2023,
title = {3D-QCNet – A pipeline for automated artifact detection in diffusion MRI images},
journal = {Computerized Medical Imaging and Graphics},
volume = {103},
pages = {102151},
year = {2023},
issn = {0895-6111},
doi = {https://doi.org/10.1016/j.compmedimag.2022.102151},
author = {Adnan Ahmad and Drew Parker and Suhani Dheer and Zahra Riahi Samani and Ragini Verma},
keywords = {Quality control, Artifacts, MRI, Diffusion MRI, Deep learning}
}



